Grid is Good: Adaptive Refinement Algorithms for Off-the-Grid Total Variation Minimization

We propose an adaptive refinement algorithm to solve total variation regularized measure optimization problems. The method iteratively constructs dyadic partitions of the unit cube based on i) the resolution of discretized dual problems and ii) on the detection of cells containing points that violate the dual constraints. The detection is based on upper-bounds on the dual certificate, in the spirit of branch-and-bound methods. The interest of this approach is that it avoids the use of heuristic approaches to find the maximizers of dual certificates. We prove the convergence of this approach under mild hypotheses and a linear convergence rate under additional non-degeneracy assumptions. These results are confirmed by simple numerical experiments.

==> axel.tex <==

To show the boundedness of the dual solutions, we need to work a bit more. The idea is again to show that the $(q_k)$ are bounded. To do so, we need three intermediate claims.

\begin{enumerate}[label=\alph*)]
\item \emph{A property of $A$ restricted to $\calV_k$.} 
Let $A_k : \calM(\calV_k) \to \R^m$ denote the restricted operators. Since the $\Omega_k$ are nested, the ranges of the $A_k$ also are: $\mathrm{ran}(A_k)\sse \mathrm{ran}(A_{k+1})$. In particular, the dimensions of them will be nondecreasing, and since they are all subspaces of $\R^m$, there must be a largest dimension $\hat{m}$. This dimension is furthermore reached in finite time. In other words, there is a subspace $V \sse \R^m$ so that for $k$ larger than some $\hat{k}$, all $A_k : \calM(\calV_k) \to V$ are surjective.

\item \emph{A property of the space $V$.} 
If $\alpha \in V^\perp$, $A^*\alpha$ vanishes on  $\cup_{k \in \N } \calV_k$. Indeed,  we have for $k \in \N$ and $\nu_k \in \calV_k$ arbitrary 
\begin{align*}
	\sprod{A^*\alpha, \nu_k} = \sprod{\alpha, A\nu_k} = 0,
\end{align*}
since $A\nu_k \in V$. Since $A^*\alpha$ is continuous, we conclude that it vanishes even on the closure $c\calV := \overline{\cup_{k \in \N} \calV_k}$.
 
\item \emph{A property of $A$ restricted to $U_\delta(c\calV)$.}  
Now, for $\delta>0$, consider the operators $$A_\delta^\perp : \calM(U_{\delta}(c\calV)^c)) \to V^\perp, \mu \mapsto \Pi_{V^\perp}A\mu,$$ where $\Pi_{V^\perp}$ is the orthogonal projection onto $V^\perp$ and  $U_\delta(c\calV)$ is the $\delta$-neighborhood of $c\calV$. The ranges are again nested, $\ran A_\delta \sse \ran A_{\delta'}$ for $\delta'<\delta$, and we may by the argument argue that for $\delta$ smaller than some $\delta_0>0$, the $A_\delta$ must map into a common space $W \sse V^\perp$. 

We now claim that $W$ must be equal to $V^\perp$. Suppose not, and let $\mu \in \calM(\Omega)$ arbitrary. Let further $\mu_\delta$ be the restriction of $\mu$ to $U_{\delta}(c\calV)^c$ -- 
that is, the measure defined via
\begin{align*}
	\sprod{\varphi,\mu_\delta} = \int_{U_{\delta}(c\calV)^c} \varphi \mathrm{d}\mu, \qquad \varphi \in \calC_0(\Omega).
\end{align*} 
We claim that $\Pi_{V^\perp} A\mu_\delta \to  \Pi_{V^\perp} A\mu$ for $\delta\to 0$. To see this, let $\alpha \in V^\perp$ be  arbitrary. To show is that $\sprod{\alpha,A\mu_\delta- A\mu} = \sprod{A^*\alpha, \mu_\delta - \mu} \to 0$. To this end, let $\epsilon>0$. Since $\alpha \in V^\perp$ vanishes on $c\calV$, and $\Omega$ is compact, there must be a $\delta>0$ with $\sup_{x\in U_{\delta}(c\calV)^c} \abs{A^*\alpha(x)} < \epsilon$. For this $\delta$, we get
\begin{align*}
	\abs{\sprod{A^*\alpha, \mu_\delta - \mu}} = \abs{\int_{U_\delta(\calV)^c} A^*\alpha \mathrm{d} \mu} \leq \epsilon \norm{\mu}_{TV}.
\end{align*}
The claim follows, and with that, $\Pi_{V^\perp} A\mu = \lim_{\delta \to 0} \Pi_{V^\perp} A\mu_\delta \in W$, since $\Pi_{V^\perp}A\mu_\delta \in W$ for small $\delta>0$. Hence, for any $\mu$, there must be $A\mu \in V+W$. Unless $W=V^\perp$, this is a contradiction to the surjectivity of $A$. 

\end{enumerate}
Now we can prove that the $q_k$ are bounded. First, the ultimate surjectivity of the $A_k$ onto $V$ and the inequality $1\geq \|A^* q_k\|_{L^\infty(\calV_k)}$, implies that the projections of the $q_k$ onto $V$, $q_k^V$ are bounded, and therefore also the $A^*q_k^V$, say $\norm{A^*q_k^V}_{L^\infty(\Omega)} \leq D$.  
 
Now let us prove that $((A^*\alpha_k)_{k\in \N})$, where $\alpha_k = q_k-q_k^V$, must be bounded on $U_\delta(c\calV)$ for any $\delta>0$. Concretely, let us show that $\norm{A^*\alpha_k}_{L^\infty(U_\delta(c\calV_\delta)^c)}\leq D+1$ for $k \geq k_\delta$. Suppose not. Then, there exists a sequence $(\xi_k)_{k \in \N} \sse U_\delta(c\calV)^c$ with $\abs{A_k^*\alpha_k(\xi_k)}> D+1$, which implies that $\abs{A_k^*q_k(\xi_k)}\geq \abs{A_k^*\alpha_k(\xi_k)} - \abs{A_k^*q_k^V(\xi_k)}> D+1-D = 1$. Since $\Omega$ is compact, a subsequence of the $\xi_k$ converge to, say, $\xi^*$. We have $\xi^* \in U_\delta(c\calV)^c$, and there must therefore exist a cell $\omega^*\ni \xi^*$ with $\omega^* \cap c \calV = \emptyset$. However, $\xi^*$ being a limit point of the $\xi_k$ means that there will be $\xi_k \in \omega^*$ for $k>k'$. Consequently, $\sup_{x\in \omega^*} \abs{A^*q_k(x)}>1$, and hence $\omega^* \in \Omega_k^*$, or one of its parents, for $k>k'$. Due to the fact that there only exists finitely many cells with a diameter smaller than $\omega^*$, any parent of $\omega^*$, and $\omega^*$,  will therefore eventually be subdivided, which is a contradiction to $c\calV \cap \omega^*=\emptyset$.

Now choose $\delta>0$ so small so that $A_\delta^\perp$ is surjective onto $V^\perp$. Then, the inequality  $\norm{A^*\alpha_k}_{L^\infty(U_\delta(\calV)^c}\leq D+1$ together with $\alpha_k \in V^\perp$  shows that $(\alpha_k)_{k \in \N}$ is bounded. Since the $q_k^V$ also were, we conclude that $(q_k)_{k \in \N}$ is.
Hence, $(q_k)_{k \in \N}$  has a converging subsequence, which we again do not relabel, and whose limit we denote $q_\infty$.

 


==> selection_processes.tex <==
\section{Further selection procedures} \label{sec:selections}

\af{In this section, let us discuss some further selection procedures that can be used. Using these will not cause us to converge faster than linear, but may still lead to a considerably slower growth rate of $\Omega_k$. This can in turn lead to the resolution of \eqref{eq:discdual} being numerically much lighter.}


\subsection{Higher order approximations}
\af{The tighter the upper-bounds $\Uk(\omega)$, the less the number of refined cells.
Hence, it can make sense to consider higher order Taylor expansions of $A^*q_k$. 
As an example, we can consider
\begin{equation} \label{eq:third_order}
\Uk(\omega) = \inf_{v \in \vertx(\omega)} \sup_{x \in \omega} \abs{A^*q_k(v)+ \sprod{\nabla A^*q_k(v),x-v}+ \frac{1}{2} \sprod{(A^*q_k)''(v)(x-v),x-v}} + \frac{1}{3!} \kappa_3(q_k,\omega)\diam(\omega)^3,
\end{equation}
where $\kappa_3(q_k,\omega)$ is a bound of the Lipschitz constant of $(A^*q_k)''$ restricted to $\omega$. If the $a_3$ are three times differentiable, the latter is given by
\begin{align*}
	\sup_{x\in \omega}  \Vert (A^*q_k)^{(3)}(x) \Vert ,
\end{align*}
where $\Vert H \Vert $ is the norm
\begin{align*}
	\vert \Vert H \Vert \vert = \sup_{\norm{u}_2, \norm{v}_2, \norm{w}_2\leq 1} H[u,v,w]
\end{align*}
of the trilinear form $H$. Again, we can use the crude bound $\kappa_3 \norm{q_k}$, or the more local approach
\begin{align*}
	\kappa_3(q_k,\omega) = \sum_{m=1}^M \abs{q_k[m]} \sup_{x\in \omega} \Vert {a_m^{(3)} (x)} \Vert .
\end{align*}
Given a way to calculate $\kappa_3(q_k,\omega)$, we may evaluate $\Uk(\omega)$ by calculating the maximum of a polynomial of degree $2$ over a $D$-dimensional cube. This can be implemented efficiently: Indeed, for each $v$, all critical points of the second degree polynomial on the cell, both in the interior and on the boundary, can easily be determined via solution of simple linear equations. Evaluating $\abs{A^*q_k(v)+ \sprod{\nabla A^*q_k(v),x-v}+ \frac{1}{2} \sprod{(A^*q_k)''(v)(x-v),x-v}}$ in these points, as well as the vertices of $\omega$, is hence enough to resolve \eqref{eq:third_order}.}


\af{Assuming that the $a_m \in C^3$, the  bound is of third order, as the following proposition shows.}


\begin{proposition} \label{prop:thirdorder}\af{ Let $\Uk(\omega)$ be as in \eqref{eq:third_order}
\begin{equation}\label{eq:bound_order_3}
    \Uk(\omega) - \frac{1}{3}\kappa_3(q_k,\omega) \diam(\omega)^3 \leq  \|A^*q_k\|_{L^\infty(\omega)} \leq \Uk(\omega).
\end{equation}
As a consequence, the resulting selection procedure satisfy  Assumption~\ref{ass:generic_refinement} and also  Assumption~\ref{ass:second_order_condition} if the sequence \\ $(\kappa_3(q_k,\omega)\diam(\omega))_{k\in \N}$ is uniformly bounded.}
\end{proposition}

\af{The approximation being of third instead of second order intuitively means that it will be tighter as the cells get small, and should therefore refine less unnecessary cells. This intuition should however be used with some cautions. Since $\kappa_3(q_k,\omega)$ might be much larger than $\kappa_2(q_k,\omega)$, the third order procedure may very well refine much more cells than the second order bound in early iterations. In Section \ref{sec:numerical}, we will see such effects in a practical example. Note however that when aiming for very high accuracies, one needs to let the cells get very small, whence the higher order upper bound might become relevant.}

%\af{A simple way to mitigate the fact that the second and third order bounds excel at different tasks is to simply define an upper bound by taking the infimum of the two.}




\begin{remark}
	\af{Using even higher order Taylor expansions, it is not hard to write down upper bounds of higher order, provided the $a_m$ are sufficiently smooth. However, from degree four and beyond, we will need to maximize polynomials of at least degree three over squares, which is not trivial. }
\end{remark}


\subsection{Lower-bounds on the gradient norm}

\af{The selection procedure can also incorporate techniques not only relying on upper bounds. As an example, we may try to leverage the fact that there for cells $\omega$ with $\omega \cap X_k \neq \emptyset$ exists a point $Xk \ni x_{k,s} \in \omega$ with $\nabla A^*q_k(x_{k,s})=0$. Hence,  $\inf_{x\in \Omega} \norm{\nabla A^*q_k(x)}_2 =0$. Consequently, it makes sense to only refine the} cells where the function $\abs{A^*q_k}$ might surpass $1$ \emph{and} where the gradient's norm $\|\nabla A^*q_k(x)\|_2$ is small. 
This can be achieved by designing a lower-bound $\Gk$ satisfying:
\begin{equation}
    \Gk \leq \inf_{x \in \omega} \norm{\nabla A^*q_k(x)}_2. \label{eq:gradRule2}
\end{equation}
We can then\af{, for any upper bound $\Uk(\omega)$,}  define a selection procedure of the form 
\begin{equation*}
    \Omega_k^\star \eqdef \{\omega \in \Omega_k \, \vert \, \Uk(\omega)  > 1 \quad \mbox{and} \quad  \Gk\leq 0\}.
\end{equation*}
\af{Under the assumption that the upper bound allows for Assumptions \ref{ass:generic_refinement} and \eqref{ass:second_order_condition}, the above will also. Indeed, if $\omega \cap X_k \neq \emptyset$, $\Gk \leq \inf_{x\in \omega} \norm{\nabla A^*q_k(x)}_2=0$, so such cells will still be in $\Omega_k^\star$. Also, the inclusion of the gradient condition surely does not make the selection procedure include any new cells, so Assumption \eqref{ass:second_order_condition} will still be satisfied.}

\af{Gradient based techniques are less sensitive to certain inaccuricies in the solution of the discretized dual problems \eqref{eq:discdual} than the ones based on upper bounds. To explain that more clearly, note that although we should have $\norm{A^*q_k}_{L^\infty(\calV_k)} \leq 1$ for all $k$ in theory, there may in practice very well instead be $\norm{A^*q_k}_{L^\infty(\calV_k)}= 1+ \epsilon$  for some small $\epsilon$, due to inaccuricies in the solution algorithm. The certificate being slightly bigger than one in a vertex will automatically cause the corresponding cell to be classified as a candidate by any upper bound procedure. If the $L^\infty(\calV_k)$ constraint in this manner is violated in many cells, the number of candidates for late iterations can explode for late iterations.}

\af{The gradient bounds do not suffer such problems: As follows from the proof of our main result , the certificates $\abs{A^*q_k}$ can, in late iterations, only be larger than one in regions where the certificate is strongly concave. Therefore, there will therefore be quite few cells where the gradient is small. Importantly, these circumstances are stable to small pertubations in the variable $q_k$.}

\af{Again, it} is possible to design relatively cheap rules for lower bounding $\inf_{x \in \omega} \norm{\nabla A^*q_k(x)}_2$. For instance, we could use one of the two following possibilities:
\begin{align}
    \Gk &= \sup_{v \in \vertx(\omega)} \norm{\nabla A^*q_k(v)}_2 - \kappa_2(q_k,\omega)\diam(\omega)\label{eq:grad1} \\
    \Gk &= \sup_{v \in \vertx(\omega)} \inf_{x \in \omega} \norm{\nabla A^*q_k(v) + (A^*q_k)''(v)(x-v)}_2 - \frac{\kappa_3(q_k,\omega)\diam(\omega)^2}{2},\label{eq:grad2}
\end{align}
where $\kappa_2$ and $\kappa_3$ are as above.
\begin{proposition} \label{prop:grad} The bounds \eqref{eq:grad1} and \eqref{eq:grad2} satisfy \eqref{eq:gradRule2}.
\end{proposition}

\af{
Both of these quantities can be again evaluated through optimization of polynomials of at most order $2$ on a square, and are hence easy to resolve.}
%(note in particular that $\norm{\nabla A^*q_k(x_0) + (A^*q_k)''(x_0)(x-x_0)}_2^2$ is a polynomial of degree $2$ with positive definite second degree term, so that its minimum on a square is attained in one of its vertices).
%This type of selection procedure allows further reducing the numerical complexity. 
%However, it is unnecessary to derive our main results. 
%In particular, it is not needed to derive an eventual linear rate of convergence, which is the best we can expect from such an algorithm based on dyadic partitions.
